Hypergraph Clustering for Finding Diverse and Experienced Groups

When forming a team or group of individuals, we often seek a balance of expertise in a particular task while at the same time maintaining diversity of skills within each group. Here, we view the problem of finding diverse and experienced groups as clustering in hypergraphs with multiple edge types. The input data is a hypergraph with multiple hyperedge types -- representing information about past experiences of groups of individuals -- and the output is groups of nodes. In contrast to related problems on fair or balanced clustering, we model diversity in terms of variety of past experience (instead of, e.g., protected attributes), with a goal of forming groups that have both experience and diversity with respect to participation in edge types. In other words, both diversity and experience are measured from the types of the hyperedges. Our clustering model is based on a regularized version of an edge-based hypergraph clustering objective, and we also show how naive objectives actually have no diversity-experience tradeoff. Although our objective function is NP-hard to optimize, we design an efficient 2-approximation algorithm and also show how to compute bounds for the regularization hyperparameter that lead to meaningful diversity-experience tradeoffs. We demonstrate an application of this framework in online review platforms, where the goal is to curate sets of user reviews for a product type. In this context, "experience" corresponds to users familiar with the type of product, and "diversity" to users that have reviewed related products.

==> content/v1-bound-beta.tex <==

\section{Calculating the minority vote threshold}\label{sec:hyperparameter}
The LP relaxation of our regularized objective can be written in the following form:
\begin{align}
\min_{\vx} \,\, & \vc^T \vx  + \beta \ve^T \vx\\
\text{s.t. } &\mA \vx \geq \vb \notag \\	
& \vx \geq 0 \notag
\end{align}
where $\beta$ is the parameter controlling the tradeoff between the two different parts of the objective. This is what is known as a parametric linear program. Previous work has looked at how to solve these types of LPs for different values of the tunable parameter $\beta$~\cite{Carstensen:1983:CPI:3119410.3119525,adler1992geometric}. Plotting out the optimal solutions to this objective as $\beta$ varies will trace out a piecewise linear, concave, increasing objective function.

\subsection{Finding $\beta$ where minority vote is no longer optimal}
We know that for $\beta>d_{max}/\Delta E$, the optimal solution to the original objective and its LP relaxation is given by minority vote. So assume we have an instance of the problem where for some $\beta_0>d_{max}/\Delta E$, so that the minority vote answer is optimal \emph{for the LP relaxation}. We would like to find the smallest value of $\beta^* \leq \beta_0$ such that the minority vote solution still is the optimal solution to the LP relaxation, i.e., for any $\beta < \beta^*$, minority vote is not longer optimal (at least for the LP). We can find this $\beta*$ by setting up and solving a related linear program.

Start with the linear programming relaxation of our objective, with parameter $\beta_0$. Abstract this as a linear program in the following form, where we assume that $\beta_0$ is now included in the vector objective function vector $\vc$:
\begin{align}
\min_{\vx} \,\, & \vc^T \vx \label{primal}\\
\text{s.t. } &\mA \vx \geq \vb \notag \\	
				& \vx \geq 0 \notag
\end{align}
%
The dual LP of~\eqref{primal} is
\begin{align}
\max_{\vx} \,\, & \vb^T \vy \label{dual}\\
\text{s.t. } &\mA^T \vy \leq \vc \notag \\	
& \vy \geq 0. \notag
\end{align}
From LP duality theory we know that if $(\vx, \vy)$ are feasible for~\eqref{primal} and~\eqref{dual} respectively, then $\vc^T \vx \leq \vb^T\vy$. If this inequality is tight, then we have in fact found an optimal primal-dual solution.

\subsection{Stability in LP solutions}
Finding $\beta^*$ amounts to answering, how long is the majority vote solution ``stable'' as the optimal solution. By running an auxiliary LP, we can exactly compute the range of $\beta$ values for which minority vote is optimal/stable. Consider a perturbation of the primal linear program:
\begin{align}
\min_{\vx} \,\, & \vc(\theta)^T \vx =  \vc^T \vx - \theta \Delta\vc^T \vx \label{p-pert}\\
\text{s.t. } &\mA \vx \geq \vb \notag \\
& \vx \geq 0 \notag
\end{align}
where $\Delta \vc$ and $\theta$ are chosen so that the \emph{new} objective function is equivalent to our clustering objective with a new value of $\beta = \beta_0 - \theta$.
If $\vx_0$ (which encodes the minority vote clustering) is the optimal solution to~\eqref{primal}, we want to know the range $\theta \in [0, \theta^+]$ such that $\vx_0$ is still optimal for~\eqref{dual}. The method for finding this $\theta^+$ is encapsulated in the theorem below.

\begin{theorem}
We can find $\theta^+$ by solving the following auxiliary linear program:
%
\begin{align}
\max_{\vy, \theta} \,\, &\theta \label{aux-primal}\\
\text{s.t. } &\mA^T \vy \leq \vc - \theta \Delta\vc  \notag \\
				& \vy \geq 0 \notag\\
				& \vb^T\vy = \vc^T \vx_0 - \theta \Delta \vc^T \vx_0 \notag\\
				& \theta \geq 0. \notag
\end{align}
\end{theorem}
\begin{proof}
Let $(\vy^*, \theta^*)$ be the optimal solution to~\eqref{aux-primal}. To see that $\theta^* = \theta^+$, note that the pair $(\vx^*, \vy^*)$ satisfies primal-dual optimality conditions for the perturbed LP~\eqref{p-pert} and its dual LP. Furthermore, it is the largest value of $\theta$ for which these primal-dual optimality conditions hold. This completes the proof.
\end{proof}


==> content/v1-intro.tex <==
\section{Introduction}
Starting in the mid-2010s, much work has focused on making machine learning algorithms more fair. Left to make decisions based solely on the training data, machine learning algorithms may make decisions which are biased against certain protected features of the demographic~\cite{mehrabi2019survey}. This work has led to the development of two lines of research: quantifying exactly what a fair algorithm is, and examining the details of fairness algorithms based on some fairness assumption. So far most of the research has focused on supervised learning. However, the 2017 seminal work~\cite{chierichetti2017fair} on fair clustering in metric space initiated a flurry of research in that direction. The concept of fairness there lied in maximizing the balance (ratio within a given cluster of number of nodes of a particular color least represented in a cluster to the number in the most represented cluster), and that concept has been explored in great length for a variety of clustering problems~\cite{chen2019proportionally,bera2019fair,ahmadian2019clustering,ahmadi2020fair,davidson2019making,kleindessner2019guarantees}. In~\cite{kleindessner2019guarantees} the notion of fair clustering developed in the aforementioned paper was extended to the graph setting, in the particular context of ratiocut spectral clustering.

On the other hand, some effort has also gone into incorporating fairness in team formation~\cite{machado2019fair}, committee selection and group recommendations~\cite{zehlike2017fa,celis2017multiwinner,aziz2019rule,stratigi2020fair}, allocation of indivisible goods~\cite{bouveret2017fair}, and crowdsourcing~\cite{basik2018fair,goel2019crowdsourcing}. Within these disciplines concepts of fairness outside the traditional proportionality constraints have been considered, such as envy-freeness, minimizing the utility of the least satisfied agent, and allocation of work assignments based on capacity to carry out work. However, while these frameworks are similar to our settings in certain aspects (having various categories as outputs, team formation, discrete assignments, group preferences, etc.) none deal with the setting of forming groups based on past experience. We fill this gap by proposing a new notion of fairness for group formation based on optimizing the experience and  of individuals within these groups with respect to group types.
\subsection{Contributions}
The contributions of this paper are listed below.
\begin{itemize}
	\item Define a new type of diversity/fairness with respect to past experiences
	\item Create and analyze a regularized categorical edge clustering objective which incorporates this definition of fairness, complete with an approximation guarantee and analysis of the effect of the regularization term
	\item Use this regularized objective to analyze a dynamical team formation process that places value on both experience within a certain field while also incentivizing a diversity of views
	\item Preparing and analyzing a host of team formation datasets from a variety of disciplines
\end{itemize}
We think the greatest contribution is this new view of fairness. While previous work has focused largely on fairness with respect to protected attributes or individual utility, here the concept of fairness is with respect to \textit{ideas} -- experiences and views which people may have developed while working on different tasks in the past -- and the way in which these ideas should be represented in future work.

\subsection{Review of categorical edge clustering}
Over the past two decades, a host of applications sprang up where the underlying network cannot be modeled by simple pairwise interactions but instead calls for multiple type of of ``higher-order" interactions that aim to capture the fundamental complexity of the network~\cite{benson2016higher}. However, few methods exist to analyze this wealth of data, and even fewer theory exists to support these methods, which opens the door for research in this direction. In particular, a fundamental problem in network analysis is clustering nodes based on the scores of some similarity function among them~\cite{fortunato2010community}. Recently, the categorical edge clustering framework was developed to fill the need for such a tool in the case where it is desirable to have clusters correspond to interaction types~\cite{amburg2020clustering}.

\xhdr{Notation}
Let $G = (V,E,C, \ell)$ be a hypergraph with labeled edges, where
$V$ is the set of nodes, 
$E$ is the corresponding set of (hyper)edges,
$C$ is a set of categories/labels, and
$\ell\colon E \rightarrow C$ maps edges to categories.
Let $k = \lvert C \rvert$ be the number of categories,
$E_c \subseteq E$ the set of edges with label $c$, and
$r$ the maximum hyperedge size in cardinality.

\xhdr{Categorical edge clustering objective}
Given $G$, we want to assign to each node one of the categories in $C$, producing a partition of the nodes into $k$ clusters. The objective function seeks to minimize the number of mistakes where a mistake is either 1) a hyperedge is placed in a cluster with color different from its one or 2) the hyperedge contains nodes which are assigned to multiple colors.
In particular, let $\clustering[i]$ be the color assigned to color $i$ under the clustering.
Define the category-mistake function $m_{\clustering}\colon E \rightarrow \{0,1\}$ by
\begin{equation}
m_{\clustering} (e) = \begin{cases} 1 & \text{ if $\clustering[i] \neq \ell(e) $ for any node $i \in e$,} \\
0 & \text{ otherwise}
\end{cases}
\end{equation}
for $e\in E.$
The \emph{Categorical Edge Label Clustering} objective is the sum of these mistakes over all the hyperedges:
\begin{equation}
\cc(\clustering) = \sum_{e \in E} m_{\clustering}(e).
\end{equation}
\xhdr{LP formulation} We can cast the above objective as an ILP in the terms below:
\begin{equation}
\label{eq:ccilp}
\begin{array}{lll}
\min & \sum_{c \in C} \sum_{e \in E_c} x_e & \\[1mm]
\text{s.t.} & \text{for all $v \in V$:} & \sum_{c = 1}^k x_v^c = k -1\\
& \text{for all $c \in C$, $e \in E_c$:} & x_v^c \leq x_e \text{ for all $v \in e$} \\
& x_v^c, x_e \in \{0,1\} &\text{for all $c \in C$, $v \in V$, $e \in E$.}
\end{array}
\end{equation}
Relaxing the binary constraints in~\eqref{eq:ccilp}
\begin{align*}
0 \leq x_v^c \leq 1,\quad 0 \leq x_e \leq 1,
\end{align*} 
the ILP becomes an LP. In the case of $k=2$ the constraint matrix is totally unimodular, so that the LP solution will be integral. However, for $k>2$ the problem is NP-hard.
\subsection{Outline of the paper}
In Section~\ref{sec:theories} we begin by formalizing the problem. We then propose a naive solution to the problem through diversity and experience scores, and observe that the simplicity of the solution leads to trivial behavior that does does not capture the complexity of experience exchange. We then present our main solution to the problem: a regularized, edge-based clustering objective that aims to keep edges of the same type together while at the same time promoting diversity in each cluster. We provide a 2-approximation algorithm for the NP-hard objective that is fast and scalable. Further analysis of the algorithm reveals that both for the original problem and the LP-based approximation algorithm, there exists a hyperparameter threshold after which the solution becomes trivial. Lastly, we wrap up section two by setting up the framework to use the regularized objective in a dynamical group forming process where the groups are reformed iteratively. We will use this framework extensively in Section\ref{sec:experiment}, where we apply it to the problem of generating a diverse set of reviews.

Next, in Section~\ref{sec:hyperparameter} we derive a range of hyperparameters below which the trivial solution is no longer optimal and more interesting behavior occurs. This allows us to fully analyze the phase transition that occurs as we vary the hyperparameters. We finish with a thorough evaluation of the algorithms on real-world datasets in Section~\ref{sec:experiment}. In particular, we demonstrate that the cost increase associated with the regularized objective is quite modest while increasing fairness in the clustering substantially. We finish with a series of experiments utilizing the dynamical framework on review datasets and online collaboration networks, finding interesting patterns reflective of experience exchange.

==> content/v1-objective.tex <==

\section{Fairness of experience through regularization}\label{sec:theories} 
In this section we arrive at the regularized approach for forming diverse and experienced group. We begin by illustrating why naive approaches do not capture the rich dynamics well. Next, we present an intuitive regularized approach than more naturally models diverse group formation. We analyze the objective and derive upper bounds on hyperparameter ranges corresponding to nontrivial behavior. Lastly, we introduce the dynamical group formation problems and derive results regarding fixed points and limit cycles of the process.

\subsection{Fairness with respect to experiences}
Most approaches to fairness have focused on defining some notion of balance within clusters to facilitate equal representation of every group in every cluster. However, this constraint seems forced in that nodes that might not share a high similarity score with each other end up in the same cluster. Our goal is to develop a framework that will reward experience with respect to a particular group while also encouraging diversity with respect to other ones. In particular, the goal will be to maximize experience within every cluster while at the same time promoting a diversity of views.
\subsection{Naive approaches: fairness through diversity and experience scores}
A first starting point for measuring experience with respect to group membership would be to count up the number of times an individual has participated in a certain group. Then the experience score of a cluster corresponding to group $c$ is simply the number of nodes which initially appeared in hyperedges of color $c$ which were then clustered into $c$. The diversity of that same cluster is then the number of nodes which appeared in hyperedges of other colors $c'\neq c$ which were clustered to $c$. Outside traditional diversity or fairness where the colors would be associated with protected classes, this model also captures the setting in which we want to form teams to complete a set of tasks based on their experience with that set of tasks. We generalize and formalize these notions below.
\subsubsection{Diversity and experience scores}
Let $d_v^c$ be any color degree score of node $v$ with respect to color $c$ (the number of hyperedges of color $c$ node $v$ appears in. Consider cluster $C(i)$ corresponding to color $i$. Then the diversity score corresponding to that color $i$ is given by $$D(i)=\sum_{v\in C(i),c\neq i}d_v^c$$ and the experience score by $$E(i)=\sum_{v\in C(i)}d_v^i.$$ Note that the diversity score puts more weight on nodes that have past experience in many types of connections. Similarly, the experience score for cluster $i$ puts more weight on nodes that have many connections of type $i$.

\subsubsection{An objective based on experience and diversity scores}
It is natural to consider the objective $$\max_Y\sum_{i\in C}[E(i)+\beta D(i)]$$
where the regularization parameter $\beta$ determines the relative importance of the diversity and experience scores. It turns out that the objective exhibits a phase transition at $\beta=1/2$. Below that threshold the optimizer is given by the majority vote algorithm which assigns every node to the majority color of all hyperedges it appears in while above the threshold it is given by the analogous minority vote approach. At the threshold we are indifferent between picking either the minority or majority vote cluster for each node. We formalize these observations in the following theorem.
\begin{theorem}
The majority vote algorithm produces an optimizer of the experience diversity objective when $\beta\geq1$ while the minority vote approach produces an optimizer when $\beta\leq 1$.

\end{theorem}
\begin{proof}
Consider node $i$ and without loss of generality suppose $d_i^1\geq\dots\geq d_i^k.$ Clustering $i$ into color 1 then gives contribution of $d_i^1+\beta\sum_{j=2}^{k}d_i^j$ while clustering to color $c\neq i$ gives contribution $d_i^c+\beta\sum_{j\neq c}d_i^j$. It is easy to see that because $d_i^1\geq\dots\geq d_i^k$ the first contribution is greater or equal to the second if and only if $\beta\leq 1$. Hence the majority vote produces an optimizer in this setting. A similar argument is used to show the analogous result for minority vote in the $\beta\geq1$ setting.
\end{proof}
Thus, although the objective is a natural starting point, it produces a trivial solution that has only two states, and no intermediate ones.
\subsection{A regularized categorical edge clustering approach to diversity}
We see that while the above objective is easy to analyze, it produces optimizers that do not capture intermediate states of diversity and experience. This happens because the diversity and experience scores always add to a constant. This observation leads us to consider objectives which do not have this property, so as to avoid another sharp phase transition. Our proposed solution is to regularize the categorical edge clustering objective with a penalty term that wants to maximize the diversity score over all clusterings. We show in the next theorem that maximizing diversity score is equivalent to minimizing the experience score. This will enable us to write the regularized objective in a compact form.
\begin{theorem}
For every choice of nonnegative $\beta$ the same optimizer that maximizes the total diversity score also minimizes the total experience score.
\end{theorem}
\begin{proof}
This is simply because for every $\beta$ the objective sums to a constant.
\end{proof}
We can now write the regularized objective as the following integer linear program:
\begin{equation}
\label{eq:ccilp}
\begin{array}{lll}
\min & \sum_{c \in C} \sum_{e \in E_c} x_e +\beta\sum_{v\in V}\sum_{c\in C}d_v^c(1-x_v^c)& \\[1mm]
\text{s.t.} & \text{for all $v \in V$:} & \sum_{c = 1}^k x_v^c = k -1\\
& \text{for all $c \in C$, $e \in E_c$:} & x_v^c \leq x_e \text{ for all $v \in e$} \\
& x_v^c, x_e \in \{0,1\} &\text{for all $c \in C$, $v \in V$, $e \in E$.}
\end{array}
\end{equation}
Here $d_v^c$ is the number of hyperedges of color $c$ node $v$ appears in. $x_e$ is the variable associated with edge $e$ and $x_v^c$ is the node-color variable associated with node $v$ and color $c$. It was shown in~\cite{amburg2020clustering} that the first constraint guarantees every node is assigned to at most 1 color, while the second constraint facilitates the coupling between the edge variables and the node-color variables.
Note that the first term in the objective is precisely the categorical edge clustering objective, which aims to cluster individuals which have interacted via a certain interaction type together. As a result, it could be used as a proxy for maximizing experience with respect to group types. The second is a regularization term which penalizes based on the sum of color $c$ degree nodes which appear in cluster $c$. So in other words, the objective penalizes having a high experience score! So we see that the two parts of the objective have competing goals. The $\beta$ parameter allows us to control the extent of the tradeoff between the two competing goals. It is easy to see that the second term is the same as the sum of the experience scores over all the nodes.

The advantage of this formulation over the diversity and experience objective discussed in the previous subsection is that clearly, the objective function no longer sums to a constant for fixed $\beta$. As a result we do not expect to see a sharp phase transition and instead the objective should model intermediate states well.

{\bf Computational considerations and an efficient algorithm with guarantees.} Since the original categorical clustering objective is NP-hard in the general case, and adding the extra regularization term generally does not make it any easier, the problem remains NP-hard, raising the need for fast approximation algorithms with guarantees.

We accomplish this through a simple LP algorithm with a basic rounding scheme as follows:
\begin{enumerate}
\item  Run the LP-relaxation of the Integer Program
\item  Go through all colors and if $x_v^c<1/2,$ then assign node $v$ to $c.$
\end{enumerate}
It turns out that this rounding scheme yields a two-approximation to the regularized objective, proved in the theorem below.
\begin{theorem}
The rounding algorithm outputs an at worst 2-approximation to the regularized objective optimal solution.
\end{theorem}
\begin{proof}
Let the relaxed solution set be $\{x_e^*,x_v^{*c}\}_{e\in E,v\in V,c\in C}$ and the corresponding rounded solution be the set $\{x_e,x_v^{c}\}_{e\in E,v\in V,c\in C}$. Let $y_v^c=1-x_v^c$ and $y_v^{*c}=1-x_v^{*c}$.
Our objective evaluated at the relaxed solution becomes $$S^*=\sum_{e}x_e^*+\beta\sum_{v\in V}\sum_{c\in C}d_v^cy_v^{*c}$$ while the rounded soluton becomes $$S=\sum_{e}x_e+\beta\sum_{v\in V}\sum_{c\in C}d_v^cy_v^{c}$$
We will show that $S\leq 2S^*$ by comparing the first and second parts of $S$ and $S^*$ respectively. Now since $x_e=1$ if and only if $x_e^*\geq1/2$ (which happens if and only if $x_v^{*c}\geq1/2$ for at least one $v$ in $e$) and $x_e=0$ otherwise, we must have $x_e\leq2x_e^*$ and thus $\sum_ex_e\leq 2\sum_ex_e^*$. Similarly, since $x_v^c=1$ ($y_v^c=0$) if and only if $x_v^{*c}\geq 1/2$ ($y_v^{c*}\leq 1/2$) and $x_v^c=0$ otherwise it follows that $y_v^c\leq2y_v^{*c}$. Thus we obtain that $\sum_{v\in V}\sum_{c\in C}d_v^cy_v^{c}\leq 2 \sum_{v\in V}\sum_{c\in C}d_v^cy_v^{*c}$. The result that $S\leq2S^*$ is now clear from the above.
\end{proof}
\subsection{Bounding the phase transition}
In this section we show that both the optimal integral solution, as well as the LP solution to the regularized objective transition from a nontrivial behavior to an extremely simple one (minority vote) for $\beta$ substantially large. This shows that the objective simplifies to a naive one in the large parameter range. We derive an analytic upper bound on the hyperparameter after which the behavior is guaranteed to be nontrivial. We will use the existence of this bound in the next section to allow us to efficiently compute a lower bound below which the solution must be nontrivial.

\subsubsection{Optimality of the integral objective}
We begin with the integral case of the problem. First, we derive a threshold for $\beta$ above which the minority vote solution is always optimal.
To begin, we start with some preliminaries. Let the regularization term for node $v$ be denoted by $$E(v,x(v))=\sum_{c\in C}d_v^c(1-x_v^c)$$
Here, $x(v)_c=x_v^c$ -- that is, $x(v)$ is the vector of color variables associated with node $v$, and the quantity represents the smallest possible increase in the regularized penalty any node can contribute to the overall objective score by moving away from the minority vote solution. Let $d_{max}=max_{i\in V}d(i)$ (the maximum degree of any node in the input network) and define $\Delta E=\min_{i\in V}\min_{x(i)}E(i,x(i))-E(i,x^{*}(i))$. Here, $x^{*}(i)$ is the color decision vector corresponding to the minority vote solution. We are now ready to define the criterion for transition to optimality of minority vote.
\begin{theorem}
The minority vote algorithm will produce an optimal solution to the fairness-regularized categorical edge clustering problem if $\beta$ is chosen so that $\beta>\frac{d_{max}}{\Delta E}$.

\end{theorem}
\begin{proof}First, the case where $\Delta E=0$ corresponds to all nodes having the same color degree with respect to each color. In this case the second part of the objective is constant regardless of the clustering. Then the optimizer will correspond to the categorical edge clustering solution, which is one of the minority vote solutions (as is any clustering when all the color degrees are equal). So we may assume $\Delta E\neq0$.
Consider node $i$ and suppose that the degree of node $i$ is $d(i).$ By definition, $d(i)\leq d_{max}$. The penalty of moving node $i$ away from its minority vote assignment is at least $\beta \Delta E$ while the penalty for violating all the hyperedges $i$ is in is at most $d_{max}$, so that if $d_{max}<\beta \Delta E$ then node $i$ will always be assigned to the minority solution. As a result all nodes in the network will also be assigned to that solution.

\end{proof}
It turns out that we can easily derive the value of $\Delta E$ as a function of the two lowest color degrees for any node in the network. In particular, let $d_v^{c'}=\min_{c}d_v^c$ and let $d_v^{c''}=\min_{c\neq c'}d_v^c$.
\begin{theorem}
$\Delta E=\min_{v\in V}d_v^{c'}-d_v^{c''}$

\end{theorem}
\begin{proof}
This is easy to see as the smallest increase in $E(v,x(v))$ from the optimal minority solution is to assign node $v$ to the \textit{second } smallest color in terms of color degree for $v$. Then we take a minimum over all the nodes to find the smallest such increase over all nodes in the network.

\end{proof}
Next, we derive a condition on $\beta$ under which node $i$ must deviate from the nonregularized solution. That is we answer the question of at what value of $\beta$ \textit{must} we see at least 1 node switch from the categorical edge clustering solution.
\begin{theorem} 
Node $i$ will switch to an assignment different from the one ($x^{ce}$) induced by optimizing the nonregularized objective if $\beta>\frac{d(i)}{\Delta E_c},$ where $\Delta E_c=\max_{x(i)}E(i,x^{ce}(i))-E(i,x(i))$
\end{theorem}
\begin{proof}
The condition in the theorem implied that $\beta \Delta E_c>d(i)$, so that node $i$ will have an incentive to deviate from the unregularized assignment since the cost of staying in the assignment is greater than violating all of the hyperedges the node is in.
\end{proof}

An immediate observation from the above results is the following corollary, which begins to categorize the transition from NP-hardness to simplicity that occurs as we increase the diversity regularization parameter $\beta$.
\begin{cor}

For $\beta = 0$, we recover our original NP-hard categorical edge clustering problem. However, when $\beta \rightarrow \infty$ the problem converges to one that is optimally solved in polynomial time by the minority vote approach.
\end{cor}
\subsubsection{Optimality in the continuous case}

In this section we show that for a large enough $\beta$, the minority vote solution solves the regularized LP optimally. This result enables us in Section~\ref{sec:hyperparameter} us to construct another LP which enables us to determine exactly what value of $\beta$ after which it is the optimal solution.

We begin by showing that the solution returned by solving the regularized part of the objective (whose nonconstant part is $-\sum_{v\in V}\sum_{c\in C}d_v^cx_v^c$) yields the minority vote solution without any rounding.

\begin{theorem}
Minimizing $-\sum_{v\in V}\sum_{c\in C}d_v^cx_v^c$ with the same constraints as the original $LP$ returns an assignment of nodes corresponding to the minority vote solution.

\end{theorem}
\begin{proof}
For any node $v$ we want $x_v^c$ to be as large as possible (i.e. 1) for colors which have high $d_v^c$. However, we are forced to have $\sum_{c\in C}x_v^c=k-1$. This means that we want to choose the variable corresponding to the color which has lowest color degree for node $v$ to be completely zero. So we want to assign $x_v^c=1$ for all but the variable corresponding to the lowest color degree of $v$ -- the one corresponding to the color of hyperedge $v$ appears in least (we break ties arbitrarily). As a result the LP returns an integral answer corresponding to the minority vote solution.
\end{proof}
We now consider the full regularized objective, and see that the threshold for optimality of minority vote is the same as in the case where we had integral constraints above.
\begin{theorem}
Suppose $\Delta E\neq 0$ (in which case the categorical edge clustering solution is a minority vote solution). If $\beta>\frac{d_{max}}{\Delta E}$ the LP will return an integral solution corresponding to minority vote.
\end{theorem}
\begin{proof}
Let $v^{*}=\arg\min_{v,d_v^{c'}\neq d_v^{c''}}d_v^{c'}-d_v^{c''}$ and suppose the node-color variables are assigned to a minority vote solution. We will examine the smallest cost of deviating from this configuration in terms of the second part of the objective to the largest gain this deviation could have on the first. A threshold of $\beta$ past which the gain is always smaller than the cost then implies optimality of the minority vote solution. Now consider a deviation from the minority vote solution such that $x_{v^*}^{c'}=\epsilon>0.$ This has a cost of at least $\beta\epsilon\Delta E$ in terms of the second part of the objective. The maximum gain this deviation could contribute in terms of the first part of the objective is $\epsilon d_{max}$ because the value of each hyperedge variable is bounded from below by the value of the node-color variables for the nodes it contains. So if $\beta$ is such that $d_{max}<\beta\Delta E$ the optimal solution is given by minority vote. 

\end{proof}

Now that we have established that there exists a threshold of $\beta$ after which minority vote is optimal both for the ILP and the LP, we provide a method to calculate the exact value at which the transition happens.
\subsubsection{A dynamical group formation framework}

The regularized objective developed and analyzed in the preceding sections allows us to cluster individuals into teams based on their past experience. However, so far this has been a one-step process. In this section, we extend the notion of team formation to a dynamical process whereby at every timestep, teams are formed based on past experience, and the current assignments then become part of the past experience at the next iteration. We derive theoretical results regarding this process in the extreme $\beta$ regimes. Further, we run the process on many real-world datasets and point out the salient features of team formation that the abstraction captures. 
\subsection{Problem setup}
Suppose we have $n$ nodes, all of which are assigned to $k$ types of tasks at the first iteration $t=0$. This corresponds to an initial assignment of employees to teams in a given year. At the next time interval $t=1$, we want to reassign the employees to tasks so as to maximize the experience they have had with these tasks while at the same time incorporating a diversity of experiences -- so that we have incentive to include people who have not worked on the task before to bring in fresh ideas, as this may increase productivity. We perform this assignment by running the regularized categorical edge clustering objective on the hypergraph $G$ induced by the work assignments at $t=0$. The hyperedges are formed around people who worked on the same task, and colored according to the task type. Before proceeding to the next reassignment, we append the hyperedges induced by the work assignment at $t=1$ to $G$. We then perform the process again at $t=2$, and continue until some time horizon $t=T$. The procedure is illustrated in Figure~\ref{fig:dynamical}
\subsubsection{Starting with a longer history}
In the above formulation, we started the dynamical process at $t=0$ with a hypergraph containing only $k$ edges. It would be more meaningful in a variety of settings to start the dynamical process from a longer history of group formation. This makes sense physically in the following context: we have observed a team formation process for some years, and starting at $t=1$ want to start following a more diverse grouping procedure. So we modify the process by starting instead with a large hypergraph representing past interactions, and make the process fair going forward.
\subsection{Looking at only a window of history}
Recent experiences may be more valuable and relevant than older ones. As a result, in constructing the history hypergraph $G$ we might only be interested in the interactions and experiences the members have had in only the $w$ most recent time intervals. We denote the graph that only keeps a window $w$ worth of history at time $t$ as $G(w,t)$. It turns out that we can obtain a lot of nice theoretical results about this setup.
\subsubsection{Dynamics in the case of $\beta=0$}
The case of no regularization corresponds to conducting the dynamical process using solely the categorical edge clustering objective. As it turns out the result is very boring, and highlights the need for diversity through regularization.
\begin{ob}
If $\beta=0$ then node will remain in the assignment given to it at time $t=1$ for all time in the absence of regularization.

\end{ob}
\begin{proof}
There is no incentive for a node to change colors after the initial clustering as this would increase the cut and the objective seeks to minimize it.
\end{proof}
Looking at this theorem through a dynamical systems perspective, we could say that this corresponds to every node being a fixed point. Indeed, the process it trivial and dull in the absence of regularization. However, it makes a lot of sense with respect to the interpretation we have been giving to the first term as incentivizing preserving experience. Indeed, the best way to build experience is to grow it by always assigning the same people to the same tasks.
\subsubsection{Dynamics in the case of $\beta\to\infty$}
As seen from the analysis in previous sections, if $\beta>d_{max}/\Delta E$ at every step of the dynamical process then the optimal solution at each step will be given by running minority vote on $G(w,t)$. Since at any given time interval $t$ a node is placed exactly into 1 hyperedge and we are considering $w$ time intervals worth of history, $d_{max}=w$ for $G(w,t)$.

We now ask the question: what are the longterm dynamics of the nodes as this process continues? We answer it in the theorem below.
\begin{theorem}

As $t\to\infty$ in the case where $\beta>d_{max}/\Delta E$, the color degree distribution corresponding to each node becomes uniform. That is if we let $d_v^c(t)$ represent the number of times that node node $v$ has been assigned to color $c$ up through time $t$, then $\lim_{t\to\infty}d_v^c(t)/d_v^{c'}(t)=1$ for all $c,c'\in C$.
\end{theorem}

\begin{proof}
For $w<k$ the longterm behavior for each node is to choose any color among the other $k-w$ colors at each step, resulting in a slow shuffling through all the possible colors available, with ties broken by choosing any of the tied colors at random with equal probabilities. When $w\geq k$ the longterm behavior for each node at each step is to choose the color that appears least among the $w$ previous assignments for the node, with ties broken randomly. As this process continues, randomly breaking ties forces the color distributions to become more uniform. In the long time limit, the distribution will become uniform with probability tending to 1.

\end{proof}
This result makes sense with respect to how we interpret the regularized part of the objective. With the contribution of the first term completely irrelevant, the second term incentivizes minorities to rise up. Indeed, the culmination of all minorities rising up is having a completely uniform distribution of colors in the longterm. Here we obtain total equality, though at the sacrifice of any semblance of experience.

==> content/v2-bound-beta.tex <==
\section{Bounding Trivial Parameter Regimes with LP Sensitivity Analysis}
\label{sec:hyperparameter}
%Our framework provides a way to balance experience and diversity in clustering, but in extremal parameter regimes it outputs solution that may entirely focus on one or the other. In this section we demonstrate how to obtain much tighter bounds on non-extremal parameter regimes based on sensitivity analysis in linear programming. 
%Our results are related to past research on bounding the optimal parameter regime for in clustering applications~\cite{gan2019graph,nowozin2009solution} adapted to apply to our fairness-regularized clustering framework.
%\subsection{Finding $\beta$ where minority vote is no longer optimal}
%
%Theorems~\ref{thm:betalarge} and~\ref{thm:betalargelp} show both our original objective and its LP relaxation return extremal (relaxed or integral) minority vote solutions when $\beta > d_\mathit{max}$.
%
 In order to find a meaningful balance between clustering based on both experience and diversity, we would ideally like to find the \emph{smallest} value of $\beta$, call it $\beta^*$, for which minority vote is optimal. Given that the objective is NP-hard in general, computing $\beta^*$ exactly may not be feasible. However, we will show that it is in fact possible to exactly the minimum value $\hat{\beta}$ for which a \emph{relaxed} minority vote solution is no longer optimal for the LP-relaxation of our objective. This has several important implications. When the minority vote clustering is unique, Theorem~\ref{thm:betalargelp} tells us that this clustering will also be optimal for the LP for large enough $\beta$. Even when it is not unique, it may still be the case (as we indeed find in our experimental results) that choosing a minority vote solution will still be optimal for the LP relaxation for large enough $\beta$. In these case, we know that $\beta^* \leq \hat{\beta}$, which allows us to rule out a wide range of parameters leading to solutions that effectively ignore the \emph{experience} part of our objective. Even in cases where an integral minority vote solution is never optimal for the LP relaxation, computing $\hat{\beta}$ provides a way to avoid parameter regimes where the LP relaxation does not simply return a \emph{relaxed} minority vote solution.


% As we will see later in our experiments, solving the LP relaxation typically provides a very close approximation to our optimal objective, and $\hat{\beta}$ provides a very useful bound in practice. 

Our approach for computing $\hat{\beta}$ is based on previous techniques for bounding the optimal parameter regime for a relaxed to solution to a clustering objective~\cite{gan2019graph,nowozin2009solution}. We have adapted these results to apply to our fairness-regularized clustering objective. This technique can also be used to the smallest value of $\beta$ for which LP relaxation of our objective will coincide with the relaxed solution to the categorical edge clustering objective, though for simplicity we focus on how to compute $\hat{\beta}$. 

\subsection{Fairness Regularization as Parametric Programming}
The LP relaxation of our regularized objective can be written abstractly in the following form
\begin{align}
\label{lp}
\min_{\vx} \,\,  \vc_e^T \vx  + \beta \vc_d^T \vx \,\, \text{ s.t. } \mA \vx \geq \vb,  \vx \geq 0 
\end{align}
where $\vx$ stores variables $\{x_e, x_v^c\}$, $\mA \vx \geq \vb$ encodes constraints given by the LP relaxation of~\eqref{eq:ccilp}, and $\vc_e, \vc_d$ denote vectors corresponding to the experience and diversity terms in our objective, respectively. Written in this format, we see that this LP-relaxation is a parametric linear program in terms of $\beta$. Standard results on parametric linear programming~\cite{adler1992geometric} guarantee that any solution to~\eqref{lp} for a fixed value of $\beta$ will in fact be optimal for a range of values $[\beta_\ell, \beta_u]$ containing $\beta$. 
%A significant amount of previous research has gone into understanding the behavior of solutions to of parametric linear programs as a parameter like $\beta$ is varied~\cite{Carstensen:1983:CPI:3119410.3119525,adler1992geometric} . 
The optimal solutions to~\eqref{lp} as a function of $\beta$ corresponds to a piecewise linear, concave, increasing curve, where each linear piece to a range of $\beta$ values for which the same feasible LP solution is optimal.

We begin by solving this LP for some value of $\beta_0 > d_\mathit{max}$, which is guaranteed to produce a solution vector $\vx_{0}$ that is either a solution to minority vote, or is at very least a relaxed form of minority vote (Theorem~\ref{thm:betalargelp}). Our goal is to find the smallest value $\hat{\beta}$ for which $\vx_{0}$ no longer optimally solves~\eqref{lp}. To do so, define $\vc = \vc_e^T \vx  + \beta \vc_d^T$ so that we can re-write objective~\eqref{lp} with $\beta = \beta_0$ as
\begin{align}
\label{primal}
\min_{\vx} \,\,  \vc^T \vx \,\, \text{ s.t. } \mA \vx \geq \vb , \vx \geq 0.
\end{align}
%The dual of this linear program is:
%\begin{align}
%\label{dual}
%\max_{\vx} \,\,  \vb^T \vy \,\, \text{ s.t. }\mA^T \vy \leq \vc,  \vy \geq 0. 
%\end{align}
 
\subsection{Stability range of the minority vote solution}
Finding $\hat{\beta}$ amounts determining how long the minority vote solution ``stable'' as the optimal solution to~\eqref{primal}. Consider a perturbation of linear program~\eqref{primal}:
\begin{align}
\label{p-pert}
\min_{\vx} \,\, & \vc(\theta)^T \vx =  \vc^T \vx - \theta \vc_d^T \vx,  \,\, \text{ s.t. } \mA \vx \geq \vb,  \vx \geq 0 
\end{align}
where  $\theta = \beta_0 - \beta$ for some $\beta< \beta_0$, so that~\eqref{p-pert} corresponds to our clustering objective with new parameter $\beta$. Since $\vx_0$ is optimal for~\eqref{primal}, it is optimal for~\eqref{p-pert} when $\theta = 0$. Solving the following linear program will tell us the range $\theta \in [0, \theta^+]$ for which $\vx_0$ is still optimal for~\eqref{p-pert}:
\begin{equation}
\label{aux-primal}
\begin{array}{ll}
\max_{\vy, \theta} \,\, \theta\,\,\text{ s.t. } &\mA^T \vy \leq \vc - \theta \vc_d \\
& \vb^T\vy = \vc^T \vx_0 - \theta \vc_d^T \vx_0 \\
& \theta \geq 0, \vy \geq 0.
\end{array}
\end{equation}
Let $(\vy^*, \theta^*)$ be the optimal solution to~\eqref{aux-primal}. The constraints in this linear program are explicitly designed so that the pair $(\vx_0, \vy^*)$ satisfy primal-dual optimality conditions for the perturbed linear program~\eqref{p-pert} and its dual, and the objective function simply indicates that we want to find the maximum value of $\theta$ such that these conditions hold. Thus, $\theta^* = \theta^+$, and $\beta = \beta_0 - \theta^+$ will be the smallest parameter value such that $\vx_0$ is optimal for the LP relaxation of our objective.



==> content/v2-intro.tex <==
\section{Introduction}
Left to make decisions based solely on training data, machine learning algorithms may make decisions that are biased or unfair towards a subset of a population~\cite{mehrabi2019survey}. This realization has led to a flurry of recent activity on fairness in algorithms, broadly seeking to address two major questions: what exactly constitutes fairness (for a given task), and how (if at all) can an algorithm efficiently achieve a given standard or fairness? Specifically within the clustering literature, fairness is typically formulated in terms of protected attributes on data points -- a cluster is fair if it exhibits a proper balance between nodes from different protected classes. The goal is then to design algorithm that optimizes a clustering objective while also adhering to constraints ensuring a balance on the protected attributes.
%
%One major focus has been to develop algorithms that form clusters that are balanced or proportional in terms of protected attributes associated with data points. 
%The key motivation of this approach is to discourage unequal treatment of members of different classes. 
%This often involves starting with an existing clustering objective and imposing a set of balance constraints for protected attributes that an algorithm should adhere to while optimizing the objective. 
This approach was initiated by Chierichetti et al.~\cite{chierichetti2017fair} in the context of clustering in metric spaces, and has been explored at a great length in related settings~\cite{chen2019proportionally,bera2019fair,ahmadian2019clustering,ahmadi2020fair,davidson2019making}, including extensions to fair and balanced clustering in graphs~\cite{kleindessner2019guarantees}. 

In this paper, we motivate and explore a new type of fairness in clustering that differs from previous approaches both in terms of the type of input data as well as the desired notion of fairness. First of all, we focus on clustering edge-labeled hypergraphs, where a hyperedge represent a set of objects (such as a group of individuals at a company) that have participated in a group interaction or experience. The hyperedge label encodes the \emph{type} or \emph{category} of interaction (e.g., a type of team project at the company). The output is then a labeled clustering, where clusters labels are chosen from the set of hyperedge labels. Regarding fairness, our goal is to form clusters whose nodes are balanced in terms of \emph{experience} and \emph{diversity}, which is distinct from (though need not be in competition with) forming balancing clusters in terms of protected attributes. By \emph{experience} we mean that a cluster with label $\ell$ should contain nodes that already have previous experience participating in hyperedges of label $\ell$. By \emph{diversity}, we mean that clusters should also include nodes that are diverse in terms of past participate in different hyperedge types. 

%Clustering based on diversity and experience should be viewed as a complementary to, rather than competing with, fair clustering based on protected attributes.
One motivating application of our framework is to fair team formation, where the goal is to assign a task to a group of people who (1) already have some level of experience working together on the given task, and (2) are diverse in terms of their previous work experience. Another application is to recommender systems, where a recommender platform may wish to show users a diversity of reviews for a certain class of products, while still maintaining a cohesive theme as much as possible.

Our mathematical framework for diverse and experienced clustering builds on a previous objective for clustering edge-labeled hypergraphs~\cite{amburg2020clustering}. This previous framework assigns nodes to labeled clusters in such a way that hyperedges of a certain label tend to be contained in a cluster with the same label. We modify this objective by adding a regularization term that additionally encourages clusters to contain nodes that have participated in many different hyperedge types. This diversity-encouraging regularization is governed by a tunable parameter $\beta \geq 0$, where $\beta  = 0$ corresponds to the original edge-labeled clustering objective.  Although the resulting objective is NP-hard in general, we design a linear programming algorithm that guarantees a 2-approximation for any choice of $\beta$. In a certain parameter regime, the objective reduces to a trivial problem with a degenerate solution. In order to guide users in selecting meaningful parameter values and avoid trivial solutions, we show how to bound the region in which non-trivial solutions occur, by leveraging previous techniques on sensitivity in linear programming. Finally, we develop and analyze a dynamic version of our objective in which groups iteratively evolve over time based on previous solutions to the regularized objective. We demonstrate the utility of our framework by applying it to team formation of users posting answers on Stack Overflow, and the task of aggregating a diverse set of reviews for categories of services and products on review sites (e.g., Yelp and Amazon).



==> content/v2-objective.tex <==
\section{Forming Clusters Based on Diversity and Experience}
We begin by introducing key notation for edge-labeled clustering, after which we analyze an approach that seems natural for clustering based on experience and diversity, but leads only to trivial solutions. We then show how a regularized version of a previous categorical edge clustering framework~\cite{amburg2020clustering} leads to the more meaningful objective that we focus on in the remainder of the paper.

%and reward clusters that avoid splitting up hyperedges. However, we also show that our objective undergoes a phase transition and a after a certain point reduces to a trivial objective. This motivates a future section on bounding the regime of meaningful parameters. Finally, we discuss a dynamic version of our framework,

\xhdr{Notation for Labeled Hypergraph Clustering}
Let $G = (V,E,C, \ell)$ be a hypergraph with labeled edges, where
$V$ is the set of nodes, 
$E$ is the set of (hyper)edges,
$L$ is a set of edge labels, and
$\ell\colon E \rightarrow L$ maps edges to labels. Let $k = \lvert L \rvert$ be the number of label, $E_c \subseteq E$ the set of edges with label $c$, and
$r$ the maximum hyperedge size in cardinality. It will often be convenient to think of hyperedge labels as corresponding to different colors, so we interchangeably refer to labels, categories, and colors. 
%
Given this input, our goal is to assign a color/label to each node. Equivalently, we form a clustering $\mathcal{C}$ in which each node is assigned to exactly one cluster, and there is exactly one cluster for each color in $L$. We wish to do this in a way that promotes both diversity (clusters have nodes from a range of colored hyperedges), and experience (a cluster with color $c$ contains nodes that have experience participating in hyperedges of color $c$). 
%Following a previous approach~\cite{amburg2020clustering}, we will always form exactly one cluster of each color.  

\subsection{Naive approaches yield trivial solutions}
We define\textit{begin by defining} two simple scores for measuring the diversity and experience corresponding to a clustering $\mathcal{C}$ of an edge-labeled hypergraph $G$. For a node $v \in V$, let $d_v^c$ be the number of hyperedges of color $c$ that node $v$ appears in. We refer to $d_v^c$ as the color degree of $v$ for color $c$. For a clustering $\mathcal{C}$, we use $\mathcal{C}(i)$ to denote the clustering with color $i \in L$. The diversity and experience scores for $\mathcal{C}(i)$ are given respectively by
\begin{equation}
\label{eq:dande}
D(i)=\sum_{v\in \mc(i),c\neq i}d_v^c\,, \hspace{.5cm} E(i)=\sum_{v\in \mc(i)}d_v^i.
\end{equation}
In words, $D(i)$ measures the extent to which nodes in cluster $i$ have participated in hyperedges that are \emph{not} color $i$. Meanwhile, $E(i)$ measures the extent to which nodes in cluster $i$ have participated in hyperedges of color $i$. A seemingly natural but naive approach for balancing experience and diversity in clustering applications is to solve the following objective:
\begin{equation}
\label{eq:naiveobj}
\max_\mc \sum_{i\in L}[E(i)+\beta D(i)].
\end{equation}
The regularization parameter $\beta$ determines the relative importance of the diversity and experience scores. It turns out that the optimal solutions to this objective are overly-simplistic, with a phase transition at $\beta=1$. Define two simple types of clusterings as follows:
\begin{itemize}
	\item \emph{Majority vote}: Node $v$ is placed in cluster $\mc(i)$ where $i = \argmax_{c \in C} d_v^c$,
	\item \emph{Minority vote}: Node $v$ is placed in cluster $\mc(i)$ where $i = \argmin_{c \in C} d_v^c$.
\end{itemize}
\begin{theorem}
	The majority vote clustering optimizes~\eqref{eq:naiveobj} for all $\beta > 1$, and minority vote optimizes the same objective for all $\beta < 1$. Both are optimal when $\beta = 1$.
\end{theorem}
\begin{proof}
	For node $i$, assume without loss of generality the colors $1, 2, \hdots k$ are ordered so that $d_i^1\geq\dots\geq d_i^k.$ Clustering $i$ with cluster 1 gives a contribution of $d_i^1+\beta\sum_{j=2}^{k}d_i^j$ to the objective, while clustering it with color $c\neq i$ gives contribution $d_i^c+\beta\sum_{j\neq c}d_i^j$. Because $d_i^1\geq\dots\geq d_i^k$, the first contribution is greater than or equal to the second if and only if $\beta\leq 1$. Hence, majority vote is optimal when $\beta \geq 1$. A similar argument proves optimality for minority vote when $\beta\geq1$.
\end{proof}
Objective~\eqref{eq:naiveobj} is easy to analyze, but produces optimizers that do not capture a meaningful balance between diversity and experience. This is essentially because a clustering will maximize the total diversity $\sum_{c \in \mc} D(c)$ if and only if it minimizes total experience $\sum_{c \in \mc} E(c)$, since these objectives sum to a constant. 

\subsection{Fairness-regularized categorical edge clustering}
We now turn a more sophisticated approach that corresponds to a regularized version of the \emph{categorical edge clustering} objective of Amburg et al.~\cite{amburg2020clustering}. In the original objective, a clustering $\mc$ receives a penalty of 1 every time a hyperedge of color $c$ is not completely contained in the cluster $\mathcal{C}(c)$. Formally, the objective is expressed as follows:
\begin{equation}
\label{obj:cec}
\min_\mc \sum_{c \in L} \sum_{e \in E_c} x_e
\end{equation}
where $x_e$ is an indicator variable equal to 1 if hyperedge $e \in E_c$ is \emph{not} contained in cluster $\mathcal{C}(c)$, but is zero otherwise. This all-or-nothing penalty encourages \emph{entire} hyperedges to be contained inside clusters of the corresponding color. For our context, this objective can be interpreted as promoting \emph{group} experience in cluster formation: if a group of people have participated together in task $c$, this is an indication they could work well together on task $c$ in the future. However, we want to avoid the scenario where groups of people endlessly work on the same type task without the benefiting from the perspective of others who have a diverse set of work experiences. Therefore, we regularize objective~\eqref{obj:cec} adding a penalty term $\beta \sum_{c \in L} E(c)$. Since the $\sum_{c \in \mathcal{C}} [E(c)+D(c)]$ is a constant, this regularization term implicitly encourages higher diversity scores $D(c)$ for each cluster $\mc(c)$. The resulting objective, which we focus on in the remainder of the paper, can be stated as an integer linear program. We'll refer to this as fairness-regularized categorical edge clustering:
\begin{equation}
\label{eq:ccilp}
\begin{array}{lll}
\min & \sum_{c \in L} \sum_{e \in E_c} x_e +\beta\sum_{v\in V}\sum_{c\in L}d_v^c(1-x_v^c) &\\[1mm]
\text{s.t.} & \text{for all $v \in V$:} & \sum_{c = 1}^k x_v^c = k -1\\
& \text{for all $c \in L$, $e \in E_c$:} & x_v^c \leq x_e \text{ for all $v \in e$} \\
& x_v^c, x_e \in \{0,1\} &\text{for all $c \in L$, $v \in V$, $e \in E$.}
\end{array}
\end{equation}
The binary variable $x_v^c$ equals $1$ if node $v$ is not assigned label $c$, and is 0 otherwise. As shown in~\cite{amburg2020clustering}, the first constraint guarantees every node is assigned to exactly 1 color, while the second constraint guarantees that if a single node $i \in e$ is not assigned to the cluster of the color of $e$, then $x_e = 1$. 
%Thus, our regularized objective inherits NP-hardness from the original problem. 

\xhdr{A polynomial-time 2-approximation algorithm} 
When $\beta = 0$, objective~\eqref{eq:ccilp} corresponds to the objective of Amburg et al.~\cite{amburg2020clustering}. Since this objective is NP-hard, our more generalized objective inherits this hardness as well. Although the optimal solution to~\eqref{eq:ccilp} may vary significantly depending on the parameter $\beta$, we develop a simple algorithm based on linear programming that enables us to obtain a 2-approximation for every value of $\beta$. The linear programming (LP) relaxation of objective~\eqref{eq:ccilp} is the linear program obtained by replacing binary constraints $x_v^c, x_e \in \{0,1\}$ with linear constraints $x_v^c, x_e \in [0,1]$. This can be solved in polynomial time, with the objective score providing a lower bound on the optimal solution to the NP-hard objective. The values of $x_v^c$ can then be \emph{rounded} into integer solutions, to produce a clustering that is within a bounded factor of the LP lower bound, and therefore within a bounded factor of optimality. Our algorithm is stated simply as follows:
% This is hacky latex. Can explore other ways to succintly give this simple algorithm.
\begin{equation}
\textbf{Algorithm 1} \hspace{.5cm} 
\begin{array}{l}
	\text{1. Run the LP-relaxation of the Integer Program}\\
	\text{2. Visit each node $v \in V$; if $x_v^c<1/2,$ then assign node $v$ to $c.$}
\end{array}
\end{equation}
We note that the first constraint in~\eqref{eq:ccilp} ensures that $x_v^c$ can only be less than $1/2$ for a single cluster.
\begin{theorem}
	For any $\beta \geq 0$, Algorithm 1 returns a 2-approximation for objective~\eqref{eq:ccilp}.
\end{theorem}
\begin{proof}
	Let the relaxed solution set be $\{x_e^*,x_v^{*c}\}_{e\in E,v\in V,c\in C}$ and the corresponding rounded solution be the set $\{x_e,x_v^{c}\}_{e\in E,v\in V,c\in C}$. Let $y_v^c=1-x_v^c$ and $y_v^{*c}=1-x_v^{*c}$.
	Our objective evaluated at the relaxed and rounded solutions respectively are
	\begin{equation}
	S^*=\sum_{e}x_e^*+\beta\sum_{v\in V}\sum_{c\in C}d_v^cy_v^{*c} \text{ and } S=\sum_{e}x_e+\beta\sum_{v\in V}\sum_{c\in C}d_v^cy_v^{c}.
	\end{equation} 
	We will show that $S\leq 2S^*$ by comparing the first and second terms of $S$ and $S^*$ respectively. For every edge $e$, $x_e=1$ if and only if $x_v^{*c}\geq1/2$ for some $v \in e$. This in turn means that $x_e^*\geq1/2$, so we would have $x_e\leq2x_e^*$. If $x_e = 0$, then $x_e\leq2x_e^*$ holds trivially. Thus, $\sum_ex_e\leq 2\sum_ex_e^*$. Similarly, since $x_v^c=1$ ($y_v^c=0$) if and only if $x_v^{*c}\geq 1/2$ ($y_v^{c*}\leq 1/2$), and $x_v^c=0$ otherwise, it follows that $y_v^c\leq2y_v^{*c}$. Thus we obtain that $\sum_{v\in V}\sum_{c\in C}d_v^cy_v^{c}\leq 2 \sum_{v\in V}\sum_{c\in C}d_v^cy_v^{*c}$.
\end{proof}

\subsection{Avoiding trivial solutions for extreme values of $\beta$}
In general, solving objective~\eqref{eq:ccilp} will provide a meaningful way to balance group experience (the first term), and diversity (the regularization). However, when $\beta \rightarrow \infty$, the objective corresponds to simply minimizing experience, i.e., maximizing diversity. We will formally show that the optimal integral solution~\eqref{eq:ccilp}, as well as the relaxed LP solution under certain conditions, transition from nontrivial behavior to trivial solutions (specifically, the minority vote clustering) when $\beta$ becomes too large. This motivates us in Section~\ref{sec:hyperparameter} to study how to bound the nontrivial parameter regime. Similarly, when $\beta$ is 0 or too close to zero, the optimal solution to~\eqref{eq:ccilp} will correspond to the vanilla categorical edge clustering problem~\cite{amburg2020clustering}, so we also consider bounds for avoiding this case.

\xhdr{Minority vote is optimal for large $\beta$}
We begin by considering a simple bound on $\beta$ above which minority vote is optimal. Let $d_\mathit{max}$ represent the largest number of edges any node participates in.
\begin{theorem}
	\label{thm:betalarge}
 For every $\beta > d_\mathit{max}$, minority vote will be optimal for~\eqref{eq:ccilp}.
\end{theorem}
\begin{proof}
	Let binary variables $\{x_e, x_v^c\}$ encode a clustering for~\eqref{eq:ccilp} that is not a minority vote solution. This means that there exists at least one node $v$ such that $x_v^c = 0$ for some color $c \neq m = \argmin_{i \in L} d_v^i$. If we move node $v$ from cluster $c$ to cluster $m$, then the regularization term in the objective would decrease (i.e. improve) by $\beta (d_v^c - d_v^{m}) \geq \beta > d_\mathit{max}$, since degrees are integer-valued and $d_v^c > d_v^{m}$. Meanwhile, the first term in the objective would increase (i.e., become worse) by at most $\sum_{e: v \in e} x_e = d_\mathit{max} < \beta$. Therefore, an arbitrary clustering that is not a minority vote solution cannot be optimal when $\beta > d_{\mathit{max}}$.
\end{proof}

% Previous approach--this works, but I feel it's much longer than necessary and often hard to follow.
%
%We begin by considering optimal solutions to the original integral objective~\eqref{eq:ccilp}. 
%Let $x$ denote an arbitrary vector of variables satisfying constraints in~\eqref{eq:ccilp}.
%% and $x(v)$ denote the set of color variables associated with not $v$, i.e., $x(v)_c=x_v^c$. 
%Let $\mathcal{M}$ denote the set of minority vote solutions (there may be many), and $x^*$ be an arbitrary solution from $\mathcal{M}$. If we denote the regularization term in~\eqref{eq:ccilp} by $E(x)=\sum_{v \in V} \sum_{c\in L}d_v^c(1-x_v^c)$, then the 
%smallest possible change in regularization term in objective~\eqref{eq:ccilp} can be expressed as:
%\begin{equation}
%\Delta E= \min_{x \notin \mathcal{M}}( E(x)-E(x^{*})),
%\end{equation}
%If $\mathcal{M} = \emptyset$, this means that all nodes have the same color degree for all colors, and thus every possible clustering is a minority vote solution. In this case, $\Delta E = 0$. Otherwise, $\Delta E > 0$.
%\begin{lemma}
%	\label{lem:betalarge}
%	Assuming $\Delta E \neq 0$, for every $\beta>\frac{d_\mathit{max}}{\Delta E}$, minority vote will produce an optimal solution to the fairness-regularized categorical edge clustering problem~\eqref{eq:ccilp}, where %d_\mathit{max}$ is the maximum number of hyperedges any edge is in.
%\end{lemma}
%\begin{proof}
%	Consider node $i$ and suppose that the degree of node $i$ is $d(i).$ By definition, $d(i)\leq d_{max}$. The penalty of moving node $i$ away from its minority vote assignment is at least $\beta \Delta E$, while the penalty for violating all the hyperedges $i$ is in is at most $d_{max}$. Since, $d_{max}<\beta \Delta E$, node $i$ will always be assigned to the minority solution.
%\end{proof}
%The bound given in this lemma is quite loose; this result should be viewed as a proof of concept. In Section~\ref{sec:hyperparameter}, we will demonstrate an approach for computing a much tighter bound.

%\xhdr{Minority vote optimality for the LP relaxation}

A slight variant of this result also holds for the LP relaxation. For a node $v \in V$, let $\mathcal{M}_v \subset L$ denote the set of minority vote clusters for $v$: $m \in \mathcal{M}_v \iff m = \argmin_{c \in L} d_v^c$. The next theorem indicates that for $\beta > d_\mathit{max}$, the LP places all ``weight'' for a node $v$ on its minority vote clusters.
\begin{theorem}
	\label{thm:betalargelp}
For every $\beta > d_\mathit{max}$, the optimal solution to the LP relaxation of~\eqref{eq:ccilp} will satisfy $\sum_{c \in \mathcal{M}_v} (1-x_v^c) = 1$ for every $v \in V$.
\end{theorem}
\begin{proof}
	Let $\{x_e, x_v^c\}$ encode an arbitrary solution to the \emph{LP relaxation} of~\eqref{eq:ccilp}, and assume specifically that it is \emph{not} a minority vote solution. For every $v \in V$ and $c \in L$, let $y_v^c = 1-x_v^c$. The $y_v^c$ variables indicate the weight or proportion of $v$ that is placed in cluster $c$, with $\sum_{c \in L} y_v^c = 1$. Since $\{x_e, x_v^c\}$ is not a minority vote solution, there exists some $v \in V$ and $j \notin \mathcal{M}_v$ such that $y_v^j = \varepsilon > 0$. We will show that as long as $\beta > d_\mathit{max}$, we could obtain a strictly better solution by moving this weight of $\varepsilon$ from cluster $j$ to a cluster in $\mathcal{M}_v$. 
	
	Choose an arbitrary $m \in \mathcal{M}_v$, and define a new set of variables $\hat{y}_v^j = 0$, $\hat{y}_v^m = y_v^m + \varepsilon$, and $\hat{y}_v^i = y_v^i$ for all other $i \notin \{m,j\}$. Define $\hat{x}_v^c = 1-\hat{y}_v^c$ for all $c \in L$. For any $u \in V$, $u \neq v$, we keep variables the same: $\hat{y}_u^c = y_u^c$ for all $c \in L$. Set edge variables $\hat{x}_e$ to minimize the LP objective subject to the $\hat{y}_c$ variables, i.e., for $c \in L$ and every $e \in E_c$, let
	\[
	\hat{x}_e = \min_{u \in V} \hat{x}_u^c \,.
	\]
	Our new set of variables simply takes the $\varepsilon$ weight from cluster $j$ and moves it to $m \in \mathcal{M}_v$. This improves the regularization term in the objective by at least $\beta \varepsilon$:
	\begin{align*}
	\beta \sum_{c \in L} d_v^c [y_v^c - \hat{y}_v^c]  &= \beta d_v^m(y_v^m - \hat{y}_v^m) + \beta d_v^j (y_v^j - \hat{y}_v^j) = -\beta d_v^m \varepsilon + \beta d_v^j \varepsilon = \beta \varepsilon (d_v^j - d_v^m) \geq \beta \varepsilon\,.
	\end{align*}
	Next, we will show that the first part of the objective increases by at most $\varepsilon d_\mathit{max}$. To see why, note that for $e \in E_j$ with $v \in e$, we have $\hat{x}_e \geq 1- \hat{y}_v^j = 1 \implies \hat{x}_e = 1$, and $x_e \geq 1-y_v^j = 1- \varepsilon$. Therefore, for $e \in E_j$, $v \in e$, we know that $\hat{x}_e - x_e = 1 - x_e \leq 1 - (1-\varepsilon) = \varepsilon$. For $e \in E_m$ with $v \in e$ we know $\hat{x}_e - x_e \leq 0$, since $\hat{x}_e = \min_{u \in V} (1- \hat{y}_u^m)$ and $x_e = \min_{u \in V} (1- y_u^m)$, but the only difference between $y_u^m$ and $\hat{y}_u^m$ variables is that $\hat{y}_v^m = y_v^m + \varepsilon \implies (1- \hat{y}_v^m) < (1-y_v^m)$. For all other edge sets $E_c$ with $c \notin \{m, j\}$, $\hat{x}_e = x_e$. Therefore,
	\begin{align*}
	\sum_{e: v \in e} [\hat{x}_e -x_e] &\leq \sum_{e \in E_j, v \in e}  [\hat{x}_e -x_e]  \leq |E_j| \cdot \varepsilon \leq  \varepsilon d_{\mathit{max}}\,.
	\end{align*}
	In other words, as long as $\beta > \varepsilon$, we can strictly improve the objective by moving around a positive weight $y_v^j = \varepsilon$ from a non-minority vote cluster $j \notin \mathcal{M}_v$ to some minority vote cluster $m \notin \mathcal{M}_v$. Therefore, at optimality, for every $v \in V$ we have $\sum_{c \in \mathcal{M}_v} y_v^c = 1$.	
\end{proof}
Theorem~\ref{thm:betalargelp} immediately implies that if the minority vote clustering is unique, meaning that each node has one color degree strictly lower than all others, then this minority vote clustering will be optimal for both the origin objective and the LP relaxation whenever $\beta > d_\mathit{max}$. Whether the optimal solution to the LP relaxation is an integral or relaxed version of minority vote, this will often correspond to a trivial solution that does not meaningfully balance diversity and experience. For this reason, in Section~\ref{sec:hyperparameter} we turn to techniques which allow us to avoid these degenerate parameter regimes when using LP relaxation techniques to solve our objective.

%We note that there do exist cases where an integral minority vote solution will never be optimal for the LP if this assumption does not hold. One can check that this will be the case for a three node complete graph where every edge has a different label. However, in many other cases, an integral minority vote solution will be optimal for the LP even if there are multiple minority vote solutions. Furthermore, Theorem~\ref{thm:betalargelp} indicates that even pathological cases, there is a regime $\beta$ values for which trivial (integral or relaxed) minority vote solutions are optimal. The condition $\beta > d_\mathit{max}$ provides simply a loose bound above which we know we will find these trivial solutions. In Section~\ref{sec:hyperparameter} we turn to techniques which allow us to avoid these degenerate parameter regimes.

\xhdr{Avoiding the non-regularized solution}
For $\beta$ values that are positive but very close to zero, the optimal solution to~\eqref{eq:ccilp} may still correspond to the optimal categorical edge clustering ($\beta = 0$) solution. In the interest of focusing on solutions that encourage a meaningful amount of diversity, we give a sufficient condition for guaranteeing when a node will deviate its $\beta = 0$ cluster assignment.

Let $x$ denote an arbitrary vector of variables satisfying constraints in~\eqref{eq:ccilp}. The contribution of node $v$ to the fairness-regularization term in our objective is given by
\begin{equation*}
E(v, x) = \sum_{c \in L} d_v^c (1- x_v^c).
\end{equation*}
 Define $X_0$ to be the set of optimal solutions to the categorical edge clustering $\beta = 0$ objective. For $x^{ce} \in X_0$, the largest possible change in the regularization term for a node $v$ among clusterings that are not $x^{ce}$ is given by
\begin{equation}
\Delta E_v(x^{ce}) =\max_{x \notin X_0}E(v,x^{ce})-E(v,x).
\end{equation}
\begin{theorem} 
Let $x^{ce} \in X_0$. For an node $v \in V$ with total degree $d(v)$, if $\beta>\frac{d(v)}{\Delta E_v}$, the optimal solution to~\eqref{eq:ccilp} will place $v$ in different cluster that the one assigned to it by $x^{ce}$,
\end{theorem}
\begin{proof}
	The condition in the theorem implies that $\beta \Delta E_v>d(v)$, meaning that node $v$ will have an incentive to deviate from the cluster assignment given by $x^{ce}$, since the cost of staying in that assignment is greater than violating all of the hyperedges the node is in.
\end{proof}


\subsection{A dynamical group formation framework}
%The regularized objective developed and analyzed in the preceding sections allows us to cluster individuals into teams based on their past experience. However, so far this has been a one-step process, where a fixed hypergraph structure is assumed. In this section, we extend the notion of team formation to a dynamical process whereby at every time-step, teams are formed based on past experience, and the current assignments then become part of the past experience at the next iteration. We derive theoretical results regarding this process in the extreme $\beta$ regimes. Further, we run the process on many real-world datasets and point out the salient features of team formation that the abstraction captures. 
In this section we introduce a dynamic variant of our framework in which we iteratively update our hypergraph based on previous a solutions to the fairness regularized clustering objective. In this way, our framework for team formation becomes a dynamical process whereby at every time-step, teams are formed based on past experience, and the current assignments then become part of the past experience at the next iteration. 
%We derive theoretical results regarding this process in the extreme $\beta$ regimes.

\xhdr{Problem setup}
Suppose we have $n$ nodes, all of which are assigned to $k$ types of tasks at the first iteration $t=0$. For example, this may correspond to an initial assignment of employees to teams in a given year. At the next time interval $t=1$, we want to reassign the employees to tasks so as to maximize the experience they have had with these tasks while at the same time incorporating a diversity of experiences -- so that we have incentive to include people who have not worked on the task before to bring in fresh ideas and perspectives. We perform this assignment by running our fairness-regularized objective on the hypergraph $G$ induced by the work assignments at $t=0$. The hyperedges are formed around people who worked on the same task, and colored according to the task type. The output clusters then become new hyperedges in an updated version of the hypergraph at time $t=1$. We then cluster the updated hypergraph again, and continually repeat this procedure until some time horizon $t=T$. The procedure is illustrated in Figure~\ref{fig:dynamical}. 

There are two slight variants of the above framework that we will employ in practice. \textbf{(1) Starting with a longer history. } First of all, we will often assume that when we begin our dynamical process at $t =0$, we are already able to draw from a history of past observed experiences, i.e., we start with a hypergraph with many labeled hyperedges.
%It would be more meaningful in a variety of settings to start the dynamical process from a longer history of group formation. 
This makes sense physically in the following context: we have observed a team formation process for some years, and starting at $t=1$ want to start following a more diverse grouping procedure. 
%So we modify the process by starting instead with a large hypergraph representing past interactions, and make the process fair going forward.
%
\textbf{(2) Looking at only a window of history.}
Recent experiences may be more valuable and relevant than older ones. As a result, in constructing the history hypergraph $G$, we might only be interested in the interactions and experiences the members have had in only the $w$ most recent time intervals. We denote the graph that only keeps a window $w$ worth of history at time $t$ as $G(w,t)$. 

\xhdr{Dynamics in the case of $\beta=0$}
The case of no regularization corresponds to conducting the dynamical process using solely the categorical edge clustering objective. This results in a trivial dynamical process: after gaining new experience from a cluster assignment at one time step, in the next time step the node has no incentive to move to a new cluster if there is no regularization term ($\beta = 0$). Therefore, it will always remain in the same cluster. 
%\begin{ob}
%	If $\beta=0$ then node will remain in the assignment given to it at time $t=1$ for all time in the absence of regularization.
%\end{ob}
%\begin{proof}
%	There is no incentive for a node to change colors after the initial clustering as this would increase the cut and the objective seeks to minimize it.
%\end{proof}
From a dynamical systems perspective, this means that every node is a fixed point. This does have a meaningful interpretation from the view that the first term in our objective provides an incentive to preserve experience. Indeed, the best way to build experience for a certain task is to always assigning the same people to the same tasks. However, this process is trivial in the absence of regularization, and does nothing to encourage diversity of past experience.

\xhdr{Dynamics in the case of $\beta\to\infty$}
As seen from the analysis in previous sections, if $\beta>d_{max}$ at every step of the dynamical process, then the optimal solution at each step will be given by running minority vote on $G(w,t)$. Since at any given time interval $t$ a node is placed exactly into 1 hyperedge and we are considering $w$ time intervals worth of history, $d_{max}=w$ for $G(w,t)$. The following theorem addresses the long-term dynamics of the nodes as this process.
\begin{theorem}
	As $t\to\infty$ in the case where $\beta>d_{max}$, the color degree distribution corresponding to each node becomes uniform. That is, if we let $d_v^c(t)$ represent the number of times that node $v$ has been assigned to color $c$ up through time $t$, then $\lim_{t\to\infty}d_v^c(t)/d_v^{c'}(t)=1$ for all $c,c'\in L$.
\end{theorem}

\begin{proof}
	For $w<k = |L|$ the long-term behavior for each node is to choose any color among the other $k-w$ colors at each step, resulting in a slow shuffling through all the possible colors available, with ties broken by choosing any of the tied colors at random with equal probabilities. When $w\geq k$ the long-term behavior for each node at each step is to choose the color that appears least among the $w$ previous assignments for the node, with ties broken randomly. As this process continues, randomly breaking ties forces the color distributions to become more uniform. In the long time limit, the distribution will become uniform with probability tending to 1.
	
\end{proof}
This result makes sense with respect to how we interpret the regularized part of the objective. With the contribution of the first term completely irrelevant, the second term incentivizes minorities to rise up. Indeed, the culmination of all minorities rising up is having a completely uniform distribution of colors in the long term. Here we obtain total equality, though at the sacrifice of any semblance of experience.

==> content/v2-related.tex <==
\xhdr{Related work}
Our work shares some similarities with previous notions of diversity in team formation~\cite{machado2019fair}, committee selection and group recommendations~\cite{zehlike2017fa,celis2017multiwinner,aziz2019rule,stratigi2020fair}, allocation of indivisible goods~\cite{bouveret2017fair}, and crowdsourcing~\cite{basik2018fair,goel2019crowdsourcing}. Within these disciplines concepts of diversity outside the traditional proportionality constraints have been considered, such as envy-freeness (cite), minimizing the utility of the least satisfied agent (cite), and allocation of work assignments based on capacity to carry out work (cite). However none of these deal with forming groups based specifically on past experience.


==> content/v3-intro.tex <==
\section{Introduction}
Left to make decisions based solely on training data, machine learning algorithms may make decisions that are biased or unfair towards a subset of a population~\cite{mehrabi2019survey}. This realization has led to a flurry of recent activity on fairness in algorithms, broadly seeking to address two major questions: what exactly constitutes fairness (for a given task), and how (if at all) can an algorithm efficiently achieve a given standard or fairness? Specifically within the clustering literature, fairness is typically formulated in terms of protected attributes on data points -- a cluster is fair if it exhibits a proper balance between nodes from different protected classes. The goal typically is to then design an algorithm that optimizes a clustering objective while also adhering to constraints ensuring a balance on the protected attributes.
This approach was initiated by Chierichetti et al.~\cite{chierichetti2017fair} in the context of clustering in metric spaces, and has been explored at a great length in related settings~\cite{chen2019proportionally,bera2019fair,ahmadian2019clustering,ahmadi2020fair,davidson2019making,kleindessner2019guarantees}. 

Although balancing protected attributes in cluster formation is applicable in many contexts, this accounts for only one notion of cluster fairness that can be meaningfully encouraged in practice. In this paper we explore a new notion of  fairness in clustering that focuses on forming groups that are \emph{experienced} and \emph{diverse} in terms of past group interactions. As a motivating example, consider a fair team formation task in which the goal is to assign a task to a group of people who (1) already have some level of experience working together on the given task, and (2) are diverse in terms of their previous work experience. As another example, a recommender system may wish to show users a diverse set of reviews for a certain class of products, while still maintaining a cohesive theme as much as possible. In other words, the set of displayed reviews should work well together in providing an accurate overview of the product category. While other alternative notions of fairness in group formation have also been considered in previous work~\cite{zehlike2017fa,celis2017multiwinner,aziz2019rule,stratigi2020fair,machado2019fair}, to our knowledge ours is the first framework that considers fair clustering based on diversity of experience.

We formalize the task of diverse and experienced group formation as a clustering problem on edge-labeled hypergraphs. In this context, a hyperedge represents a set of objects (such as a group of individuals) that have participated in a group interaction or experience. The hyperedge label encodes the \emph{type} or \emph{category} of interaction (e.g., a type of team project). The output is then a labeled clustering, where cluster labels are chosen from the set of hyperedge labels. The goal is to form clusters whose nodes are balanced in terms of \emph{experience} and \emph{diversity}. By \emph{experience} we mean that a cluster with label $\ell$ should contain nodes that already have previous experience participating in hyperedges of label $\ell$. By \emph{diversity}, we mean that clusters should also include nodes that are diverse in terms of past participation in different hyperedge types. 

Our mathematical framework for diverse and experienced clustering builds on a previous objective for clustering edge-labeled hypergraphs~\cite{amburg2020clustering}. This previous framework assigns nodes to labeled clusters in such a way that hyperedges of a certain label tend to be contained in a cluster with the same label. We modify this objective by adding a regularization term that additionally encourages clusters to contain nodes that have participated in many different hyperedge types. This diversity-encouraging regularization is governed by a tunable parameter $\beta \geq 0$, where $\beta  = 0$ corresponds to the original edge-labeled clustering objective.  Although the resulting objective is NP-hard in general, we design a linear programming algorithm that guarantees a 2-approximation for any choice of $\beta$. We show that in a certain parameter regime, the objective reduces to a trivial problem with a degenerate solution. In order to guide users in selecting meaningful parameter values and avoid trivial solutions, we show how to bound the region in which non-trivial solutions occur, by leveraging previous techniques on sensitivity in linear programming. Finally, we develop and analyze a dynamic version of our objective in which groups iteratively evolve over time based on previous solutions to the regularized objective. We demonstrate the utility of our framework by applying it to team formation of users posting answers on Stack Overflow, and the task of aggregating a diverse set of reviews for categories of services and products on review sites (e.g., Yelp and Amazon).



==> content/v4-intro.tex <==
\section{Fair Clustering and Group Formation}
Left to make decisions based solely on training data, machine learning
algorithms may make decisions that are biased or unfair towards a subset of a
population~\cite{barocas2016big,chouldechova2017fair,corbett2018measure}.
There are now a variety of algorithmic fairness techniques to combat this
issue~\cite{corbett2017algorithmic,kleinberg2018algorithmic,mehrabi2019survey},
which broadly seek to address two overarching questions: what constitutes
fairness (for a given task), and how (if at all) can an algorithm efficiently
guarantee fairness? For the broad task of clustering, fairness is
typically formulated in terms of protected attributes on data points --- a
cluster is ``fair'' if it exhibits a proper balance between nodes from different
protected classes. The goal is then to design an algorithm that
optimizes a classical clustering objective while also adhering to constraints
ensuring a balance on the protected attributes. This approach has been applied
to a variety of clustering objectives and types of data
(e.g., point cloud or graph data)~\cite{ahmadi2020fair,ahmadian2019correlation,ahmadian2019clustering,bera2019fair,chen2019proportionally,chierichetti2017fair,davidson2019making,kleindessner2019guarantees}.

Although balancing protected attributes in clusters is broadly applicable, this
accounts for only one notion of cluster fairness that can be meaningfully
encouraged in practice. In this paper we explore a new notion of fairness in
clustering that focuses on forming groups that are \emph{diverse} and
\emph{experienced} in terms of past group interactions. As a motivating example,
consider a fair team formation task in which the goal is to assign a task to a
group of people who (1) already have some level of experience working together
on the given task, and (2) are diverse in terms of their previous work
experience. As another example, a recommender system may want to display a
diverse yet cohesive set of reviews for a certain class of products. In other
words, the set of displayed reviews should work well together in providing an
accurate overview of the product category. There are alternative fair group
formation
algorithms~\cite{aziz2019rule,celis2018multiwinner,kleinberg2018team,machado2019fair,stratigi2020fair,zehlike2017fa},
but these do not focus on diversity of experience, which has long been of
interest in sociology, psychology, and business
management~\cite{forsyth2018group,homan2008facing,jackson1995diversity,levi2015group}.


Here, we formalize diverse and experienced group formation as a
clustering problem on edge-labeled hypergraphs. In this context, a hyperedge
represents a set of objects (such as a group of individuals) that have
participated in a group interaction or experience. The hyperedge label encodes
the \emph{type} or \emph{category} of interaction (e.g., a type of team
project). The output is then a labeled clustering of nodes, where cluster labels
are chosen from the set of hyperedge labels. The goal is to form clusters whose
nodes are balanced in terms of \emph{experience} and \emph{diversity}. By
\emph{experience} we mean that a cluster with label $\ell$ should contain nodes
that have previously participated in hyperedges of label $\ell$.
By \emph{diversity}, we mean that clusters should also include nodes
that have participated in other hyperedge types.

Our mathematical framework for diverse and experienced clustering builds on an
existing objective for clustering edge-labeled
hypergraphs~\cite{amburg2020clustering}. This objective encourages cluster
formation in such a way that hyperedges of a certain label tend to be contained
in a cluster with the same label, similar to (chromatic) correlation
clustering~\cite{bansal2004correlation,bonchi2015chromatic}. We add a
regularizer to this objective that encourages clusters to contain nodes that
have participated in many different hyperedge types. This diversity-encouraging
regularization is governed by a tunable parameter $\beta \geq 0$, where $\beta =
0$ corresponds to the original edge-labeled clustering objective. Although the
resulting objective is NP-hard in general, we design a linear programming
algorithm that guarantees a 2-approximation for any choice of $\beta$. We show
that certain values of this hyperparameter reduce to extremal solutions with
closed-form solutions where just diversity or just experience is encouraged. In
order to guide a meaningful hyperparameter selection, we show how to bound the
region in which non-extremal solutions occur, leveraging linear programming
sensitivity techniques. Finally, we develop and analyze a dynamic version of our
objective in which groups iteratively evolve over time based on previous
solutions to the regularized objective. We demonstrate the utility of our
framework by applying it to team formation of users posting answers on Stack
Overflow, and the task of aggregating a diverse set of reviews for categories of
establishments and products on review sites (e.g., Yelp and Amazon).



==> content/v5-intro.tex <==
\section{Clustering and Diverse Group Formation}



In this paper we explore a new notion of diversity in
clustering that focuses on forming groups that are \emph{diverse} and
\emph{experienced} in terms of past group interactions. As a motivating example,
consider a diverse team formation task in which the goal is to assign a task to a
group of people who (1) already have some level of experience working together
on the given task, and (2) are diverse in terms of their previous work
experience. As another example, a recommender system may want to display a
diverse yet cohesive set of reviews for a certain class of products. In other
words, the set of displayed reviews should work well together in providing an
accurate overview of the product category. There are alternative diverse group
formation
algorithms~\cite{aziz2019rule,celis2018multiwinner,kleinberg2018team,machado2019fair,stratigi2020fair,zehlike2017fa},
but these do not focus on diversity of experience, which has long been of
interest in sociology, psychology, and business
management~\cite{forsyth2018group,homan2008facing,jackson1995diversity,levi2015group}.


Here, we formalize diverse and experienced group formation as a
clustering problem on edge-labeled hypergraphs. In this context, a hyperedge
represents a set of objects (such as a group of individuals) that have
participated in a group interaction or experience. The hyperedge label encodes
the \emph{type} or \emph{category} of interaction (e.g., a type of team
project). The output is then a labeled clustering of nodes, where cluster labels
are chosen from the set of hyperedge labels. The goal is to form clusters whose
nodes are balanced in terms of \emph{experience} and \emph{diversity}. By
\emph{experience} we mean that a cluster with label $\ell$ should contain nodes
that have previously participated in hyperedges of label $\ell$.
By \emph{diversity}, we mean that clusters should also include nodes
that have participated in other hyperedge types.

Our mathematical framework for diverse and experienced clustering builds on an
existing objective for clustering edge-labeled
hypergraphs~\cite{amburg2020clustering}. This objective encourages cluster
formation in such a way that hyperedges of a certain label tend to be contained
in a cluster with the same label, similar to (chromatic) correlation
clustering~\cite{bansal2004correlation,bonchi2015chromatic}. We add a
regularizer to this objective that encourages clusters to contain nodes that
have participated in many different hyperedge types. This diversity-encouraging
regularization is governed by a tunable parameter $\beta \geq 0$, where $\beta =
0$ corresponds to the original edge-labeled clustering objective. Although the
resulting objective is NP-hard in general, we design a linear programming
algorithm that guarantees a 2-approximation for any choice of $\beta$. We show
that certain values of this hyperparameter reduce to extremal solutions with
closed-form solutions where just diversity or just experience is encouraged. In
order to guide a meaningful hyperparameter selection, we show how to bound the
region in which non-extremal solutions occur, leveraging linear programming
sensitivity techniques. Finally, we develop and analyze a dynamic version of our
objective in which groups iteratively evolve over time based on previous
solutions to the regularized objective. We demonstrate the utility of our
framework by applying it to team formation of users posting answers on Stack
Overflow, and the task of aggregating a diverse set of reviews for categories of
establishments and products on review sites (e.g., Yelp and Amazon).

This work is related to the fair clustering literature, and we explore the connections in detail in the following subsection.
\subsection{Relation to fair clustering}
Left to make decisions based solely on training data, machine learning
algorithms may make decisions that are biased or unfair towards a subset of a
population~\cite{barocas2016big,chouldechova2017fair,corbett2018measure}.
There are now a variety of algorithmic fairness techniques to combat this
issue~\cite{corbett2017algorithmic,kleinberg2018algorithmic,mehrabi2019survey},
which broadly seek to address two overarching questions: what constitutes
fairness (for a given task), and how (if at all) can an algorithm efficiently
guarantee fairness? For the broad task of clustering, fairness is
typically formulated in terms of protected attributes on data points --- a
cluster is ``fair'' if it exhibits a proper balance between nodes from different
protected classes. The goal is then to design an algorithm that
optimizes a classical clustering objective while also adhering to constraints
ensuring a balance on the protected attributes. This approach has been applied
to a variety of clustering objectives and types of data
(e.g., point cloud or graph data)~\cite{ahmadi2020fair,ahmadian2019correlation,ahmadian2019clustering,bera2019fair,chen2019proportionally,chierichetti2017fair,davidson2019making,kleindessner2019guarantees}. These approaches are similar to our notion of diverse clustering as in both cases, the resulting clusters are more heterogeneous with respect to node attributes. While the primary attribute addressed in fair clustering is the protected status of a data point, in our case it is the diversity of that point with respect to prior participation in group types. The authors would go so far as to suggest that our notion of diverse team formation actually defines a novel type of {\it fairness} with respect to past experience and backgrounds, as the resulting diverse groups avoid polarization based on prior experience. For some, this notion might seem controversial. However, the interpretation one gives for the output of the algorithms we provide does not detract from their usefulness in forming teams that balance diversity with expertise.

==> content/v6-intro.tex <==
\section{Clustering and Diverse Group Formation}
In this paper we explore a new notion of diversity in
clustering that focuses on forming groups that are \emph{diverse} and
\emph{experienced} in terms of past group interactions. As a motivating example,
consider a diverse team formation task in which the goal is to assign a task to a
group of people who (1) already have some level of experience working together
on the given task, and (2) are diverse in terms of their previous work
experience. As another example, a recommender system may want to display a
diverse yet cohesive set of reviews for a certain class of products. In other
words, the set of displayed reviews should work well together in providing an
accurate overview of the product category. There are alternative diverse group
formation
algorithms~\cite{aziz2019rule,celis2018multiwinner,kleinberg2018team,machado2019fair,stratigi2020fair,zehlike2017fa},
but these do not focus on diversity of experience, which has long been of
interest in sociology, psychology, and business
management~\cite{forsyth2018group,homan2008facing,jackson1995diversity,levi2015group}.

{\color{blue} Consider an alternative order?
\begin{itemize}
	\item Broad importance and history of team formation
	\item Previous work has looked at algorithms for diversity in team formation
	\item However, diversity in terms of past experience has been important in sociology, psychology, and business, but algorithms for this haven't been very well studied.
	\item Therefore, in this paper we explore a new algorithmic framework for forming groups that are \emph{diverse} and \emph{experienced} in terms of past group interactions.
	\item As an example...
\end{itemize}
}


Here, we formalize diverse and experienced group formation as a
clustering problem on edge-labeled hypergraphs. In this context, a hyperedge
represents a set of objects (such as a group of individuals) that have
participated in a group interaction or experience. The hyperedge label encodes
the \emph{type} or \emph{category} of interaction (e.g., a type of team
project). The output is then a labeled clustering of nodes, where cluster labels
are chosen from the set of hyperedge labels. The goal is to form clusters whose
nodes are balanced in terms of \emph{experience} and \emph{diversity}. By
\emph{experience} we mean that a cluster with label $\ell$ should contain nodes
that have previously participated in hyperedges of label $\ell$.
By \emph{diversity}, we mean that clusters should also include nodes
that have participated in other hyperedge types.

Our mathematical framework for diverse and experienced clustering builds on an
existing objective for clustering edge-labeled
hypergraphs~\cite{amburg2020clustering}. This objective encourages cluster
formation in such a way that hyperedges of a certain label tend to be contained
in a cluster with the same label, similar to (chromatic) correlation
clustering~\cite{bansal2004correlation,bonchi2015chromatic}. We add a
regularizer to this objective that encourages clusters to contain nodes that
have participated in many different hyperedge types. This diversity-encouraging
regularization is governed by a tunable parameter $\beta \geq 0$, where $\beta =
0$ corresponds to the original edge-labeled clustering objective. Although the
resulting objective is NP-hard in general, we design a linear programming
algorithm that guarantees a 2-approximation for any choice of $\beta$. We show
that certain values of this hyperparameter reduce to extremal solutions with
closed-form solutions where just diversity or just experience is encouraged. In
order to guide a meaningful hyperparameter selection, we show how to bound the
region in which non-extremal solutions occur, leveraging linear programming
sensitivity techniques. Finally, we develop and analyze a dynamic version of our
objective in which groups iteratively evolve over time based on previous
solutions to the regularized objective. We demonstrate the utility of our
framework by applying it to team formation of users posting answers on Stack
Overflow, and the task of aggregating a diverse set of reviews for categories of
establishments and products on review sites (e.g., Yelp and Amazon).

\subsection{Relation to fair clustering}
Our work on diversity in clustering is related to the recent research on algorithmic fairness and fair clustering, which we briefly review. Left to make decisions based solely on training data, machine learning
algorithms may make decisions that are biased or unfair towards a subset of a
population~\cite{barocas2016big,chouldechova2017fair,corbett2018measure}.
There are now a variety of algorithmic fairness techniques to combat this
issue~\cite{corbett2017algorithmic,kleinberg2018algorithmic,mehrabi2019survey},
which broadly seek to address two overarching questions: what constitutes
fairness (for a given task), and how (if at all) can an algorithm efficiently
guarantee fairness? For the broad task of clustering, fairness is
typically formulated in terms of protected attributes on data points --- a
cluster is ``fair'' if it exhibits a proper balance between nodes from different
protected classes. The goal is then to design an algorithm that
optimizes a classical clustering objective while also adhering to constraints
ensuring a balance on the protected attributes. This approach has been applied
to a variety of clustering objectives and types of data
(e.g., point cloud or graph data)~\cite{ahmadi2020fair,ahmadian2019correlation,ahmadian2019clustering,bera2019fair,chen2019proportionally,chierichetti2017fair,davidson2019making,kleindessner2019guarantees}. These approaches are similar to our notion of diverse clustering, since in both cases, the resulting clusters are more heterogeneous with respect to node attributes. While the primary attribute addressed in fair clustering is the protected status of a data point, in our case it is the diversity of that point with respect to prior participation in group types. In this way, our work could be viewed or applied as a way to encourage an alternative notion of fairness in clustering. Clusters in our framework are \emph{fair} in the sense that they represent many different work backgrounds and previous experiences, rather than being restricted to a select few types of individuals. 
%At the same time, there are many other reasons why one may wish to form diverse clusters in a dataset, and we expect our framework to be applicable beyond just providing an alternative notion of clustering fairness. 
Nevertheless, we expect our techniques for regularized hypergraph clustering to be useful beyond simply providing an alternative notion of fairness for certain applications. We therefore present our approach as a general framework for clustering with \emph{diversity}, as there are many reasons why one may wish to organize a dataset into clusters that are diverse with respect to past experience.


%There are many reasons one may wish to form clusters in a dataset that are diverse in terms of previous group participation, so we broadly present our approach as a framework for diversity in clustering.


%The authors would go so far as to suggest that our notion of diverse team formation actually defines a novel type of {\it fairness} with respect to past experience and backgrounds, as the resulting diverse groups avoid polarization based on prior experience. For some, this notion might seem controversial. However, the interpretation one gives for the output of the algorithms we provide does not detract from their usefulness in forming teams that balance diversity with expertise.
